Probing sunspots with two-skip time-distance helioseismology

Previous helioseismology of sunspots has been sensitive to both the structural and magnetic aspects of sunspot structure. We aim to develop a technique that is insensitive to the magnetic component so the two aspects can be more readily separated. We study waves reflected almost vertically from the underside of a sunspot. Time-distance helioseismology was used to measure travel times for the waves. Ray theory and a detailed sunspot model were used to calculate travel times for comparison. It is shown that these large distance waves are insensitive to the magnetic field in the sunspot. The largest travel time differences for any solar phenomena are observed. With sufficient modeling effort, these should lead to better understanding of sunspot structure.

==> bibfiles <==
This is BibTeX, Version 0.99d (TeX Live 2017)
The top-level auxiliary file: paper_comb.aux
The style file: aa.bst
I couldn't open database file fred.bib
---line 88 of file paper_comb.aux
 : \bibdata{fred
 :              ,duvall}
I'm skipping whatever remains of this command
I found no database files---while reading file paper_comb.aux
Warning--I didn't find a database entry for "Schunker13"
Warning--I didn't find a database entry for "Lindsey10"
Warning--I didn't find a database entry for "Gizon09"
Warning--I didn't find a database entry for "Moradi10"
Warning--I didn't find a database entry for "Chou00"
Warning--I didn't find a database entry for "Braun87"
Warning--I didn't find a database entry for "Cameron08"
Warning--I didn't find a database entry for "Liang13"
Warning--I didn't find a database entry for "Duvall95"
Warning--I didn't find a database entry for "Chou09"
Warning--I didn't find a database entry for "Schou12"
Warning--I didn't find a database entry for "Duvall13"
Warning--I didn't find a database entry for "Duvall03"
Warning--I didn't find a database entry for "McQuillin85"
Warning--I didn't find a database entry for "Bracewell65"
Warning--I didn't find a database entry for "Jefferies94"
Warning--I didn't find a database entry for "Kosovichev97"
Warning--I didn't find a database entry for "Braun98"
Warning--I didn't find a database entry for "PrzSheCal15aa"
Warning--I didn't find a database entry for "MorCal08ab"
Warning--I didn't find a database entry for "NewCal10aa"
Warning--I didn't find a database entry for "KhoCol08aa"
Warning--I didn't find a database entry for "JurBelSch15aa"
Warning--I didn't find a database entry for "SchFle98aa"
Warning--I didn't find a database entry for "SchFle03aa"
Warning--I didn't find a database entry for "DeuGou84aa"
Warning--I didn't find a database entry for "Bog97aa"
Warning--I didn't find a database entry for "TraBriRic14aa"
Warning--I didn't find a database entry for "Cal07aa"
Warning--I didn't find a database entry for "SchCal06aa"
Warning--I didn't find a database entry for "CalMor13aa"
Warning--I didn't find a database entry for "MorCalPrz15aa"
Warning--I didn't find a database entry for "RijMorPrz15aa"
Warning--I didn't find a database entry for "Cally09"
Warning--I didn't find a database entry for "Felipe16"
Warning--I didn't find a database entry for "Felipe17"
(There were 2 error messages)


==> ref_report <==
09/01/2018

Dr Tom L., Jr. Duvall

duvall@mps.mpg.de
Our Ref. : AA/2017/32424

Dear Tom,

The manuscript entitled :

"Probing sunspots with two-skip time-distance helioseismology"

was submitted to a referee (Doug Braun) who recommends publication following minor revision (see enclosed report).

Please make the requested improvements and send us the revised version (two pdf files: one in referee format and the other in printer format) at your earliest convenience. Instructions for resubmitting can be found at address https://mms-aanda.obspm.fr/is/aa/resubmit_a_paper.php. Your author ID number is 22487.

Also make sure that the figure and table captions are formatted in accordance with the A&A instructions (see http://www.aanda.org/index.php?option=com_content&view=article&id=136&Itemid=200&lang=en_GB.utf8%2C+en_GB.UT#paper_organisation and the current A&A macro for examples).

- In your cover letter, please indicate precisely all the changes made in the revised version,
- Mark all the changes clearly (using boldface) in your manuscript.

The final acceptance letter will give you the exact acceptance date as well as instructions for sending your paper to the publisher. Please do not send your manuscript to the publisher before receiving the notice of acceptance.

With best regards,

Hardi Peter 
A&A Editor 
-------------------
Referee report

The referee, Doug Braun, waives anonymity.

This work describes a set of well planned and executed measurements and models of two-skip time-distance measurements through a sunspot derived with HMI Dopplergrams. The results are novel, interesting, and quite plausible. They expand upon and complement prior work in this long-standing, but still timely, sub-field of local helioseismology. Consequently, it is my opinion this work should be published in Astronomy and Astrophysics. I have only a few relatively minor queries and suggestions.

1) I am very interested in the use of the fixed-width phase-speed filter described here in section 2 (as used in Duvall and Hanasoge 2013). Specifically, I wonder if the authors have compared two-skip phase (and envelope) times between this filter and more "standard" phase-speed filters, as was done for supergranulation in the aforementioned work. As in that work, the results here are compared (at least in a general way) to ray-theory expectations which do not include the effects of filters, so the potential dependence on filter parameters is relevant. I bring this up because the two-skip phase times reported seem (at least to me) surprisingly high (even allowing for the factor of 2 in the two-way measurements) for this large range of skip distances. There are perhaps scant published measurements using the standard filters, but see Braun and Birch 2008 Sol Phys, 251, 267, figure 5a which shows the trend for umbral phase times vs phase-speed at fixed frequencies, and also Fig!
 8 for th
e ridge filter at n=4 which is comparable to the mode set used in this work.

2) As a minor side note to (1), I'd like to suggest the authors state explicitly the central phase-speed (say, in km/s or micro-Hertz if using nu/L) of the filter used. I found the sentence (in section 2) stating "A phase-speed filter... transmits both the 1st and 2nd skip over the range and distances used (\Delta = 12 - 24 deg)." to be somewhat confusing, since, for example the 1-skip distance seems to vary from about 6 to 12 degrees.

3) The issue of filters also comes up in relation to prior controversies regarding whether the "two-skip" measurements are (or are not) twice the sum of the inward and outward "one-skip" times which use the signal within the spot (e.g. see Zhao and Kosovichev 2006, ApJ, 643, 1317 who claim they agree when using standard phase-speed filters). Consequently, at least I would be interested in the answer how much this holds true for the measurements in this work (could be beyond the scope here, but I am still interested...) noting that the strong scattering modeled here could also play a role in all this.

4) Another minor point, but in Fig 4, the frequency spacing of the plots seems to vary (i.e. with finer steps around 3 mHz and courser steps around 4.5 mHz). The caption suggests a set of Gaussians with a step of 0.25 mHz is used, which seems not quite consistent with these plots, unless I have severely misconstrued what was done here).

5) There is a substantial offset in both the phase and envelope times for the (quiet-Sun subtracted) results shown in Figure 5 at the edges of the plots, which suggest there are travel-time shifts extending beyond the penumbra. Perhaps the authors could comment in this. I am curious as the spatial extent of this possible plateau.

6) In the discussion regarding the results of Figure 7, I am curious as to the percentage of ray paths eliminated by the filtering of anomalous second-skip distances, so as to help gauge the general agreement shown with observations.

7) In the numbered points summarizing Fig 7, item (4) on p. 7 refers to "The equivalent time phase speed Wilson depression..." which seems to be a little garbled. Later the authors use "the equivalent phase and group speed thermal depths of the Wilson depression." which seems somewhat clearer.

8) The idea, discussed in the concluding remarks, of comparing numerical models with "magnetic" and/or "thermal" components turned on and off is a good one, but also has some track record. A courtesy citation to the recent work of Felipe and colleagues (e.g 2016, ApJ, 829, 67 and 2017 A&A, 604, A126) would perhaps be nice (there are likely other references that I also ought to be aware of...).


==> response <==
24/01/2018
duvall@mps.mpg.de
Ref. : AA/2017/32424

Dear Hardi, 

The manuscript entitled :
"Probing sunspots with two-skip time-distance helioseismology"
has been revised.  The detailed responses to the referee's points are
included below.

Best regards,
Tom Duvall

-------------------


1) I am very interested in the use of the fixed-width phase-speed filter described here in section 2 (as used in Duvall and Hanasoge 2013). Specifically, I wonder if the authors have compared two-skip phase (and envelope) times between this filter and more "standard" phase-speed filters, as was done for supergranulation in the aforementioned work. As in that work, the results here are compared (at least in a general way) to ray-theory expectations which do not include the effects of filters, so the potential dependence on filter parameters is relevant. I bring this up because the two-skip phase times reported seem (at least to me) surprisingly high (even allowing for the factor of 2 in the two-way measurements) for this large range of skip distances. There are perhaps scant published measurements using the standard filters, but see Braun and Birch 2008 Sol Phys, 251, 267, figure 5a which shows the trend for umbral phase times vs phase-speed at fixed frequencies, and also Fig!
 8 for th
e ridge filter at n=4 which is comparable to the mode set used in this work.

It is a good point that the times measured are somewhat larger than some
previous results.  It would be a useful project for future work to compare
the results for different filters and different techniques (time-distance
and holography).  But we did not do this in the present work.  And it is
a fairly expensive proposition to redo the analysis with different filters.
In the previous work mentioned above, we felt that a much larger signal
was obtained by using broad filters (in phase speed) because scattering
was occurring between wavenumbers up to 1/size of the features involved
(in that case supergranules).  If one makes the filter too narrow, the
correlated signal is lost.  We suspect that a similar effect may be present
in the current case.  We chose the present filter as it is wide enough
to capture the signal for both the range of phase speeds within the distance
range used and also potential scattering.  And we do obtain a larger signal
than that obtained from narrow phase speed filters.

2) As a minor side note to (1), I'd like to suggest the authors state explicitly the central phase-speed (say, in km/s or micro-Hertz if using nu/L) of the filter used. I found the sentence (in section 2) stating "A phase-speed filter... transmits both the 1st and 2nd skip over the range and distances used (\Delta = 12 - 24 deg)." to be somewhat confusing, since, for example the 1-skip distance seems to vary from about 6 to 12 degrees.

The central phase speed of 141 km/s is now mentioned in the filter
description.  Also the 12-24 deg is specified as the 1st skip distance.

3) The issue of filters also comes up in relation to prior controversies regarding whether the "two-skip" measurements are (or are not) twice the sum of the inward and outward "one-skip" times which use the signal within the spot (e.g. see Zhao and Kosovichev 2006, ApJ, 643, 1317 who claim they agree when using standard phase-speed filters). Consequently, at least I would be interested in the answer how much this holds true for the measurements in this work (could be beyond the scope here, but I am still interested...) noting that the strong scattering modeled here could also play a role in all this.

We would also be interested in the answer to this question.  We attempted
to use the Doppler signal in the umbra to do center-to-annulus travel times.
But the Doppler signal in the umbra is compromised.  It has very large
spikes.  It seems to have something to do with the large darkness of this
spot.  We were hoping this could be improved by deconvolving the scattered
light from the filtergrams before making the Doppler signal.  But in fact this
made it worse.  It would seem that there is some saturation of the Zeeman
signal in the umbra that is adversely affecting the calculated Doppler
signal.  See Fig. 23 and accompanying discussion in
Couvidat et. al (2016, Sol. Physics 291, 1887).  

4) Another minor point, but in Fig 4, the frequency spacing of the plots seems to vary (i.e. with finer steps around 3 mHz and courser steps around 4.5 mHz). The caption suggests a set of Gaussians with a step of 0.25 mHz is used, which seems not quite consistent with these plots, unless I have severely misconstrued what was done here).

Sorry about that.  We meant to redo the analysis with the constant frequency
spacing but never got around to it.  We think the analysis is fine.  
The caption has been changed to reflect the analysis.

5) There is a substantial offset in both the phase and envelope times for the (quiet-Sun subtracted) results shown in Figure 5 at the edges of the plots, which suggest there are travel-time shifts extending beyond the penumbra. Perhaps the authors could comment in this. I am curious as the spatial extent of this possible plateau.

Some discussion of this point has been added at the end of section 2.
The crux is that it is uncertain whether this result comes from poor
horizontal resolution or is a real effect.  The extensions of the map
would be addressed in future work.

6) In the discussion regarding the results of Figure 7, I am curious as to the percentage of ray paths eliminated by the filtering of anomalous second-skip distances, so as to help gauge the general agreement shown with observations.

We have included the fraction of points excluded for each panel of Fig. 7 in
the caption for Figure 7.

7) In the numbered points summarizing Fig 7, item (4) on p. 7 refers to "The equivalent time phase speed Wilson depression..." which seems to be a little garbled. Later the authors use "the equivalent phase and group speed thermal depths of the Wilson depression." which seems somewhat clearer.

We have modified the relevant sentence in keeping with the referee's suggestion.

8) The idea, discussed in the concluding remarks, of comparing numerical models with "magnetic" and/or "thermal" components turned on and off is a good one, but also has some track record. A courtesy citation to the recent work of Felipe and colleagues (e.g 2016, ApJ, 829, 67 and 2017 A&A, 604, A126) would perhaps be nice (there are likely other references that I also ought to be aware of...).

We have included these references and two earlier ones in the discussion
of this point.

